Status Report on Global Pulsar-Timing-Array Efforts to Detect Gravitational Waves

The stability of the spin of pulsars and the precision with which these spins can be determined, allows many unique tests of interest to physics and astrophysics. Perhaps the most challenging and revolutionary of these, is the detection of nanohertz gravitational waves. An increasing number of efforts to detect and study long-period gravitational waves by timing an array of pulsars have been ongoing for several decades and the field is moving ever closer to actual gravitational-wave science. In this review article, we summarise the state of this field by presenting the current sensitivity to gravitational waves and by reviewing recent progress along the multiple lines of research that are part of the continuous push towards greater sensitivity. We also briefly review some of the most recent efforts at astrophysical interpretation of the most recent GW estimates derived from pulsar timing.

==> PTAs.tex <==
\begin{table}
\begin{tabular}{llcclrl}
  \hline
  PTA      & Telescope        & $f_{\rm c}$      & BW            & Timespan  & Ref.\\
           &                  & (MHz)            & (MHz)         &           &     \\
  \hline
  EPTA     & Effelsberg (EFF) & 1380, 2487, 4857 & 240, 300, 500 & 1996--    & \citet{eab+23}\\
           & Lovell$^1$ (JBO) & 1532             & 512           & 2009--    &     \\
           & Nan{\c{c}}ay (NRT)& 1484, 1854, 2154, 2539& 512     & 2004--    &     \\
           & Sardinia (SRT)   & 357, 1396        & 105, 500      & 2014--    &     \\
           & Westerbork (WSRT)& 350, 1380, 2273  & 80, 160, 160  & 1999--2015&     \\
           & LEAP             & 1396             & 128           & 2012--    & \citet{bjk+16}\\
           & LOFAR            & 148.9            & 78.1          & 2012--    & \citet{dvt+20}\\
  \\%\hline
  InPTA    & GMRT             & 400, 1360        & 200           & 2018--    & \citet{tnr+22}\\
   %        & Ooty (ORT)       &                  &               &           &     \\

  \\%\hline
  NANOGrav$^2$& Arecibo (AO)  & 327, 433, 1456, 2052&50, 24, 600, 460& 2004--2020& \citet{aaa+23a}\\
           & Green Bank (GBT) & 820, 1518        & 180, 640      & 2004--    &     \\
           & VLA              & 1520, 3000       & 800, 1700     & 2015--    &     \\
           & CHIME            & 600              & 400           & 2019--    & \citet{cab+21}\\
  \\%\hline
  PPTA     & Parkes (PKS)     & 2368$^3$         & 3328          & 2004--    & \citet{zrk+23}\\
  \\%\hline
  %IPTA     & All of the above &                  &               &           &     \\
  %\hline
  MPTA     & MeerKAT          & 1284             & 856           & 2019--    & \citet{msb+23}\\
  \\%\hline
  CPTA     & FAST             & 1250             & 500           & 2019--    & \citet{xcg+23}\\
  \hline
 \end{tabular}
\caption{Characteristics of PTA observations. For each PTA the different participating observatories
  are given, along with the current observing frequencies and maximal bandwidths in the different
  observing bands. The time span corresponds to the range of dates over which PTA observations were
  carried out at the observatories, including with older systems that are not detailed in this
  table. Unless otherwise specified, the first reference given for a PTA refers to  all telescopes of that PTA. The first four PTAs in this list (EPTA, InPTA, NANOGrav and PPTA) are all members of the IPTA, which also has a data-sharing agreement with the MPTA. \\ $^1$:
  For PSR~J1713+0747, the Jodrell Bank Observatory also provided data from the Mark II
  telescope. The observation's characteristics are identical to those listed above.\\ $^2$: For NANOGrav, the quoted bandwidths are the \emph{usable} bandwidth, accounting for RFI excision.\\ $^3$: The PPTA presently uses an ultra-wide-bandwidth receiver with continuous frequency coverage from 704 to 4032 MHz. In practice they split up this bandpass in eight sub-bands with center frequencies ranging from 736 to 3312 MHz.}
\label{tab:PTAs}
\end{table}


==> pulsars.tex <==
\begin{table}
 %\begin{tabular}{llrrrrccccccc}
  \begin{tabular}{lrrrrccccccc}
    \hline
    %J-name & B-name & Period (ms) & DM & P$_b$ & S1400 & EPTA & InPTA & NANOGrav & PPTA & CPTA &
    %MPTA
    Name & Period & DM & $P_{\rm b}$ & $S_{1400}$  & \multicolumn{7}{c}{Observed by}\\
    (J2000) & (ms) & (pc/cm$^3$) & (days) & (mJy) & EPTA & InPTA & NANOGrav & PPTA & CPTA & MPTA
    & LOFAR \\
    \hline
J0023+0923   &  3.05 & 14.3 & 0.1 & 0.7 & - & - & V & - & V & - & -  \\
J0030+0451   &  4.87 &  4.3 & --  & 1.1 & V & - & V & V & V & V & V  \\
J0034$-$0534 &  1.88 & 13.8 & 1.6 & 0.2 & - & - & - & - & V & - & V  \\
J0125$-$2327 &  3.68 &  9.6 & --  & 2.5 & - & - & - & V & - & V & -  \\
J0154+1833   &  2.37 & 19.8 & --  & 0.1 & - & - & - & - & V & - & -  \\
J0218+4232   &  2.32 & 61.3 & 2.0 & 0.9 & - & - & - & - & V & - & V  \\
J0340+4130   &  3.30 & 49.6 & --  & 0.3 & - & - & V & - & V & - & -  \\
J0406+3039   &  2.61 & 49.4 & 7.0 & --  & - & - & V & - & V & - & -  \\
J0407+1607   & 25.70 & 35.6 &669.1& 0.4 & - & - & - & - & - & - & V  \\
J0437$-$4715 &  5.76 &  2.6 & 5.7 &150.2& - & V & V & V & - & V & -  \\
J0509+0856   &  4.06 & 38.3 & 4.9 & 1.5 & - & - & V & - & V & - & -  \\
J0557+1551   &  2.56 &102.6 & 4.8 & --  & - & - & V & - & - & - & -  \\
J0605+3757   &  2.73 & 20.9 &55.7 & --  & - & - & V & - & V & - & -  \\
J0610$-$2100 &  3.86 & 60.7 & 0.3 & 0.7 & - & - & V & - & - & V & -  \\
J0613$-$0200 &  3.06 & 38.8 & 1.2 & 2.3 & V & V & V & V & V & V & -  \\
J0614$-$3329 &  3.15 & 37.1 &53.6 & 0.7 & - & - & V & V & - & V & -  \\
J0621+1002   & 28.85 & 36.6 & 8.3 & 1.7 & - & - & - & - & V & - & V  \\
J0636$-$3044 &  3.95 & 15.5 & --  & 1.5 & - & - & - & - & - & V & -  \\
J0636+5128   &  2.87 & 11.1 & 0.1 & 1.0 & - & - & V & - & V & - & -  \\
J0645+5158   &  8.85 & 18.2 & --  & 0.3 & - & - & V & - & V & - & V  \\
J0709+0458   & 34.43 & 44.3 & 4.4 & 0.3 & - & - & V & - & - & - & -  \\
J0711$-$6830 &  5.49 & 18.4 & --  & 2.6 & - & - & - & V & - & V & -  \\
J0732+2314   &  4.09 & 44.7 &30.2 & 0.7 & - & - & - & - & V & - & -  \\
J0740+6620   &  2.89 & 15.0 & 4.8 & 1.1 & - & - & V & - & - & - & V  \\
J0751+1807   &  3.48 & 30.2 & 0.3 & 1.4 & V & V & - & - & V & - & V  \\
J0824+0028   &  9.86 & 34.5 &23.2 & 0.5 & - & - & - & - & V & - & -  \\
J0900$-$3144 & 11.11 & 75.7 &18.7 & 3.8 & V & - & - & V & - & V & -  \\
J0931$-$1902 &  4.64 & 41.5 & --  & 0.5 & - & - & V & - & - & V & -  \\
J0952$-$0607 &  1.41 & 22.4 & 0.3 & --  & - & - & - & - & - & - & V  \\
J0955$-$6150 &  2.00 &160.9 &24.6 & 0.6 & - & - & - & - & - & V & -  \\
J1012$-$4235 &  3.10 & 71.7 &38.0 & 0.3 & - & - & V & - & - & V & -  \\
J1012+5307   &  5.26 &  9.0 & 0.6 & 3.8 & V & V & V & - & V & - & V  \\
J1017$-$7156 &  2.34 & 94.2 & 6.5 & 1.1 & - & - & - & V & - & V & -  \\
J1022+1001   & 16.45 & 10.3 & 7.8 & 3.9 & V & V & V & V & - & V & V  \\
J1024$-$0719 &  5.16 &  6.5 & --  & 1.5 & V & - & V & V & V & V & V  \\
J1036$-$8317 &  3.41 & 27.1 & 0.3 & 0.5 & - & - & - & - & - & V & -  \\
J1045$-$4509 &  7.47 & 58.1 & 4.1 & 2.7 & - & - & - & V & - & V & -  \\
J1101$-$6424 &  5.11 &207.4 & 9.6 & 0.3 & - & - & - & - & - & V & -  \\
J1103$-$5403 &  3.39 &103.9 & --  & 0.4 & - & - & - & - & - & V & -  \\
J1125$-$5825 &  3.10 &124.8 &76.4 & 1.0 & - & - & - & - & - & V & -  \\
J1125$-$6014 &  2.63 & 52.9 & 8.8 & 1.3 & - & - & - & V & - & V & -  \\
J1125+7819   &  4.20 & 12.0 &15.4 & 1.1 & - & - & V & - & - & - & V  \\
J1216$-$6410 &  3.54 & 47.4 & 4.0 & 1.2 & - & - & - & - & - & V & -  \\
J1300+1240$^a$& 6.22 & 10.2 &25.3 & 0.4 & - & - & - & - & - & - & V  \\
J1312+0051   &  4.23 & 15.3 &38.5 & 0.2 & - & - & V & - & - & - & -  \\
J1327$-$0755 &  2.68 & 27.9 & 8.4 & 0.2 & - & - & - & - & - & V & -  \\
J1327+3423   & 41.51 &  4.2 & --  & --  & - & - & - & - & V & - & -  \\
J1400$-$1431 &  3.08 &  4.9 & 9.5 & 0.2 & - & - & - & - & - & - & V  \\
\hline
\end{tabular}
  \caption{MSPs that are being timed as part of a PTA experiment. Listed are the J2000 name of the
    pulsar, its pulse period, interstellar dispersion measure, orbital period (if any), measured
    flux density at 1.4\,GHz and which PTAs it is observed by ('V' indicates the pulsar is part of
    the array, '-' indicates it is not). Values were taken from the ATNF Pulsar Catalogue \citep{mhth05}, \citet{aaa+23a} or from \citet{flm+23} in the case of PSR~J1327+3423. The source lists from the various observing campaigns were taken from the references cited in Section~\ref{ssec:Data} $^a$: PSR~J1300+1240 is also referred to as PSR~B1257+12.}
 \label{tab:PSRs}
 \end{table}


\begin{table}
 %\begin{tabular}{llrrrrccccccc}
  \begin{tabular}{lrrrrccccccc}
    \hline
    %J-name & B-name & Period (ms) & DM & P$_b$ & S1400 & EPTA & InPTA & NANOGrav & PPTA & CPTA &
    %MPTA
    Name & Period & DM & $P_{\rm b}$ & $S_{1400}$  & \multicolumn{7}{c}{Observed by}\\
    (J2000) & (ms) & (pc/cm$^3$) & (days) & (mJy) & EPTA & InPTA & NANOGrav & PPTA & CPTA & MPTA
    & LOFAR \\
    \hline
J1421$-$4409 &  6.39 &  54.6 & 30.7 & 1.3 & - & - & - & - & - & V & -  \\
J1431$-$5740 &  4.11 & 131.4 &  2.7 & 0.4 & - & - & - & - & - & V & -  \\
J1435$-$6100 &  9.35 & 113.8 &  1.4 & 0.3 & - & - & - & - & - & V & -  \\
J1446$-$4701 &  2.20 &  55.8 &  0.3 & 0.5 & - & - & - & V & - & V & -  \\
J1453+1902   &  5.79 &  14.1 &  --  & 0.2 & - & - & V & - & V & - & -  \\
J1455$-$3330 &  7.99 &  13.6 & 76.2 & 0.7 & V & - & V & - & - & V & -  \\
J1525$-$5545 & 11.36 & 127.0 &  1.0 & 0.4 & - & - & - & - & - & V & -  \\
J1543$-$5149 &  2.06 &  51.0 &  8.1 & 0.8 & - & - & - & - & - & V & -  \\
J1544+4937   &  2.16 &  23.2 &  0.1 & --  & - & - & - & - & - & - & V  \\
J1545$-$4550 &  3.58 &  68.4 &  6.2 & 1.1 & - & - & - & V & - & V & -  \\
J1547$-$5709 &  4.29 &  95.7 &  3.1 & 0.3 & - & - & - & - & - & V & -  \\
J1552+5437   &  2.43 &  22.9 &  --  & --  & - & - & - & - & - & - & V  \\
J1600$-$3053 &  3.60 &  52.3 & 14.3 & 2.4 & V & V & V & V & - & V & -  \\
J1603$-$7202 & 14.84 &  38.0 &  6.3 & 2.5 & - & - & - & V & - & V & -  \\
J1614$-$2230 &  3.15 &  34.5 &  8.7 & 1.1 & - & - & V & - & - & V & -  \\
J1629$-$6902 &  6.00 &  29.5 &  --  & 1.0 & - & - & - & - & - & V & -  \\
J1630+3734   &  3.32 &  14.2 & 12.5 & --  & - & - & V & - & V & - & -  \\
J1640+2224   &  3.16 &  18.4 &175.5 & 0.5 & V & - & V & - & V & - & V  \\
J1643$-$1224 &  4.62 &  62.4 &147.0 & 3.8 & - & V & V & V & V & V & -  \\
J1652$-$4838 &  3.79 & 188.2 &  --  & 0.9 & - & - & - & - & - & V & -  \\
J1653$-$2054 &  4.13 &  56.5 &  1.2 & 0.6 & - & - & - & - & - & V & -  \\
J1658+3630   & 33.03 &   3.0 &  3.0 & --  & - & - & - & - & - & - & V  \\
J1658$-$5324 &  2.44 &  30.8 &  --  & 0.4 & - & - & - & - & - & V & -  \\
J1705$-$1903 &  2.48 &  57.5 &  --  & 0.6 & - & - & V & - & - & V & -  \\
J1708$-$3506 &  4.51 & 146.8 &149.1 & 1.5 & - & - & - & - & - & V & -  \\
J1710+4923   &  3.22 &   7.1 &  --  & --  & - & - & - & - & V & - & -  \\
J1713+0747   &  4.57 &  16.0 & 67.8 & 8.3 & V & V & V & V & V & V & V  \\
J1719$-$1438 &  5.79 &  36.8 &  0.1 & 0.4 & - & - & V & - & - & V & -  \\
J1721$-$2457 &  3.50 &  48.2 &  --  & 0.6 & - & - & - & - & - & V & -  \\
J1730$-$2304 &  8.12 &   9.6 &  --  & 4.0 & V & - & V & V & - & V & V  \\
J1732$-$5049 &  5.31 &  56.8 &  5.3 & 2.1 & - & - & - & - & - & V & -  \\
J1737$-$0811 &  4.18 &  55.3 & 79.5 & 1.1 & - & - & - & - & - & V & -  \\
J1738+0333   &  5.85 &  33.8 &  0.4 & 0.3 & V & - & V & - & V & - & V  \\
J1741+1351   &  3.75 &  24.2 & 16.3 & 0.3 & - & - & V & V & V & - & -  \\
J1744$-$1134 &  4.08 &   3.1 &  --  & 2.6 & V & V & V & V & V & V & V  \\
J1745+1017   &  2.65 &  24.0 &  0.7 & 0.5 & - & - & V & - & V & - & -  \\
J1747$-$4036 &  1.65 & 152.9 &  --  & 1.5 & - & - & V & - & - & V & -  \\
J1751$-$2857 &  3.92 &  42.8 &110.7 & 0.5 & V & - & V & - & - & V & -  \\
J1756$-$2251 & 28.46 & 121.2 &  0.3 & 1.1 & - & - & - & - & - & V & -  \\
J1757$-$5322 &  8.87 &  30.8 &  0.5 & 1.2 & - & - & - & - & - & V & -  \\
J1801$-$1417 &  3.63 &  57.3 &  --  & 1.5 & V & - & - & - & - & V & -  \\
J1802$-$2124 & 12.65 & 149.6 &  0.7 & 0.7 & - & - & V & - & - & V & -  \\
J1804$-$2717 &  9.34 &  24.7 & 11.1 & 0.4 & V & - & - & - & - & - & -  \\
J1811$-$2405 &  2.66 &  60.6 &  6.3 & 1.3 & - & - & V & - & - & V & -  \\
J1824$-$2452 &  3.05 & 119.9 &  --  & 2.3 & - & - & - & V & - & - & -  \\
J1825$-$0319 &  4.55 & 119.6 & 52.6 & 0.2 & - & - & - & - & - & V & -  \\
J1832$-$0836 &  2.72 &  28.2 &  --  & 0.9 & - & - & V & V & V & V & -  \\
J1843$-$1113 &  1.85 &  60.0 &  --  & 0.1 & V & - & V & - & V & V & -  \\
J1853+1303   &  4.09 &  30.6 &115.7 & 0.5 & - & - & V & - & V & - & V  \\
J1857+0943$^b$& 5.36 &  13.3 & 12.3 & 5.0 & V & V & V & V & V & - & V  \\
\hline
\end{tabular}
  \caption{MSPs that are being timed as part of a PTA experiment. Continued from
    Table~\ref{tab:PSRs}. $^b$: PSR~J1857+0943 is also referred to as PSR~B1855+09.}
 \label{tab:PSRs2}
 \end{table}


\begin{table}
 %\begin{tabular}{llrrrrccccccc}
  \begin{tabular}{lrrrrccccccc}
    \hline
    %J-name & B-name & Period (ms) & DM & P$_b$ & S1400 & EPTA & InPTA & NANOGrav & PPTA & CPTA &
    %MPTA
    Name & Period & DM & $P_{\rm b}$ & $S_{1400}$ & \multicolumn{7}{c}{Observed by}\\
    (J2000) & (ms) & (pc/cm$^3$) & (days) & (mJy) & EPTA & InPTA & NANOGrav & PPTA & CPTA & MPTA
    & LOFAR \\
    \hline
J1902$-$5105 &  1.74 &  36.3 &  2.0 & 1.0 & - & - & - & V & - & V & -  \\
J1903+0327   &  2.15 & 297.5 & 95.2 & 0.6 & - & - & V & - & V & - & -  \\
J1903$-$7051 &  3.60 &  19.7 & 11.1 & 1.0 & - & - & - & - & - & V & -  \\
J1909$-$3744 &  2.95 &  10.4 &  1.5 & 1.8 & V & V & V & V & - & V & -  \\
J1910+1256   &  4.98 &  38.1 & 58.5 & 0.7 & V & - & V & - & V & - & -  \\
J1911$-$1114 &  3.63 &  31.0 &  2.7 & 1.0 & - & - & - & - & V & - & V  \\
J1911+1347   &  4.63 &  31.0 &  --  & 0.9 & V & - & V & - & V & - & -  \\
J1918$-$0642 &  7.65 &  26.6 & 10.9 & 0.6 & V & - & V & - & V & V & V  \\
J1923+2515   &  3.79 &  18.9 &  --  & 0.2 & - & - & V & - & V & - & V  \\
J1933$-$6211 &  3.54 &  11.5 & 12.8 & 1.0 & - & - & - & V & - & V & -  \\
J1939+2134$^c$& 1.56 &  71.0 &  --  &13.9 & - & V & V & V & - & - & -  \\
J1944+0907   &  5.19 &  24.4 &  --  & 2.1 & - & - & V & - & V & - & V  \\
J1946+3417   &  3.17 & 110.2 & 27.0 & 0.9 & - & - & V & - & V & - & -  \\
J1946$-$5403 &  2.71 &  23.7 &  0.1 & 0.4 & - & - & - & - & - & V & -  \\
J1955+2908$^d$& 6.13 & 104.5 &117.3 & 1.0 & - & - & V & - & V & - & V  \\
J2010$-$1323 &  5.22 &  22.2 &  --  & 0.7 & - & - & V & - & V & V & -  \\
J2017+0603   &  2.90 &  23.9 &  2.2 & 0.2 & - & - & V & - & V & - & -  \\
J2019+2425   &  3.94 &  17.2 & 76.5 & 0.3 & - & - & - & - & V & - & -  \\
J2022+2534   &  2.65 &  53.7 &  --  &  -- & - & - & - & - & V & - & -  \\
J2033+1734   &  5.95 &  25.1 & 56.3 & 0.3 & - & - & V & - & V & - & -  \\
J2039$-$3616 &  3.28 &  24.0 &  5.8 & 0.5 & - & - & - & - & - & V & -  \\
J2043+1711   &  2.38 &  20.7 &  1.5 & 0.1 & - & - & V & - & V & - & V  \\
J2051$-$0827 &  4.51 &  20.7 &  0.1 & 2.8 & - & - & - & - & - & - & V  \\
J2124$-$3358 &  4.93 &   4.6 &  --  & 4.5 & V & V & V & V & - & V & -  \\
J2129$-$5721 &  3.73 &  31.8 &  6.6 & 1.0 & - & - & - & V & - & V & -  \\
J2145$-$0750 & 16.05 &   9.0 &  6.8 & 5.5 & - & V & V & V & V & V & V  \\
J2150$-$0326 &  3.50 &  20.7 &  --  & 0.5 & - & - & - & - & V & V & -  \\
J2214+3000   &  3.12 &  22.5 &  0.4 & 0.5 & - & - & V & - & V & - & -  \\
J2222$-$0137 & 32.82 &   3.3 &  2.4 & 0.9 & - & - & - & - & - & V & V  \\
J2229+2643   &  2.98 &  22.7 & 93.0 & 0.8 & - & - & V & - & V & V & -  \\
J2234+0611   &  3.58 &  10.8 & 32.0 & 0.5 & - & - & V & - & V & - & -  \\
J2234+0944   &  3.63 &  17.8 &  0.4 & 1.9 & - & - & V & - & V & V & -  \\
J2241$-$5236 &  2.19 &  11.4 &  0.1 & 1.8 & - & - & - & V & - & V & -  \\
J2302+4442   &  5.19 &  13.8 &125.9 & 1.4 & - & - & V & - & V & - & V  \\
J2317+1439   &  3.45 &  21.9 &  2.5 & 0.6 & - & - & V & - & V & V & V  \\
J2322+2057   &  4.81 &  13.4 &  --  & 0.3 & V & - & V & - & V & V & -  \\
J2322$-$2650 &  3.46 &   6.1 &  0.3 & 0.2 & - & - & - & - & - & V & -  \\
\hline
\end{tabular}
  \caption{MSPs that are being timed as part of a PTA experiment. Continued from
    Table~\ref{tab:PSRs}. $^c$: PSR~J1939+2134 is also referred to as PSR~B1937+21. $^d$: PSR~J1955+2908
    is also referred to as PSR~B1953+29.}
 \label{tab:PSRs3}
 \end{table}

